MRRR-based Eigensolvers for Multi-core Processors and Supercomputers

The real symmetric tridiagonal eigenproblem is of outstanding importance in numerical computations; it arises frequently as part of eigensolvers for standard and generalized dense Hermitian eigenproblems that are based on a reduction to tridiagonal form. For its solution, the algorithm of Multiple Relatively Robust Representations (MRRR or MR3 in short) - introduced in the late 1990s - is among the fastest methods. To compute k eigenpairs of a real n-by-n tridiagonal T, MRRR only requires O(kn) arithmetic operations; in contrast, all the other practical methods require O(k^2 n) or O(n^3) operations in the worst case. This thesis centers around the performance and accuracy of MRRR.

==> Makefile <==

FILES = thesis.tex \
        thesis.bib \
        abstract.tex \
        acknowledgments.tex \
        chapter01a.tex \
        chapter02a.tex \
        chapter02b.tex \
        chapter03a.tex \
        chapter03b.tex \
        chapter04a.tex \
        chapter04b.tex \
        chapter04c.tex \
        chapter05a.tex \
        chapter05b.tex \
        conclusions.tex \
        appendixa.tex \
        appendixb.tex \
        appendixc.tex \
        appendixd.tex \
        appendixe.tex 

thesis.pdf: $(FILES) 
	latex thesis
	bibtex thesis
	latex thesis
	latex thesis
	dvips -D600 thesis.dvi -o
	ps2pdf thesis.ps thesis.pdf

.PHONY: clean
clean:
	rm -f thesis.ps *~ *.aux *.log *.bbl *.nst

